Transfer Q-learning

Time-inhomogeneous finite-horizon Markov decision processes (MDP) are frequently employed to model decision-making in dynamic treatment regimes and other statistical reinforcement learning (RL) scenarios. These fields, especially healthcare and business, often face challenges such as high-dimensional state spaces and time-inhomogeneity of the MDP process, compounded by insufficient sample availability which complicates informed decision-making. To overcome these challenges, we investigate knowledge transfer within time-inhomogeneous finite-horizon MDP by leveraging data from both a target RL task and several related source tasks. We have developed transfer learning (TL) algorithms that are adaptable for both batch and online $Q$-learning, integrating valuable insights from offline source studies. The proposed transfer $Q$-learning algorithm contains a novel {\em re-targeting} step that enables {\em cross-stage transfer} along multiple stages in an RL task, besides the usual {\em cross-task transfer} for supervised learning. We establish the first theoretical justifications of TL in RL tasks by showing a faster rate of convergence of the $Q^*$-function estimation in the offline RL transfer, and a lower regret bound in the offline-to-online RL transfer under stage-wise reward similarity and mild design similarity across tasks. Empirical evidence from both synthetic and real datasets is presented to evaluate the proposed algorithm and support our theoretical results.

==> extra_macro.tex <==
%\RequirePackage{amssymb}
\RequirePackage{amsthm,amsmath,amsfonts,bbm}

%%
%% Figures and tables
%%
\usepackage{caption}
\usepackage{subcaption}

\usepackage{multirow}

\usepackage{graphicx}
\graphicspath{{figs/}}

\usepackage{stmaryrd} % for \llbracket and \rrbracket


\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}

%--------------------------------
%
%  Boldfaces in Letters
%
% \newcommand{\bfm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bfm}[1]{\ensuremath{\boldsymbol{#1}}} % bm

\def\bzero{\bfm 0}
\def\bone{\bfm 1}
\def\bbone{\mathbbm{1}} % package bm

\def\ba{\bfm a}   \def\bA{\bfm A}  \def\AA{\mathbb{A}}
\def\bb{\bfm b}   \def\bB{\bfm B}  \def\BB{\mathbb{B}}
\def\bc{\bfm c}   \def\bC{\bfm C}  \def\CC{\mathbb{C}}
\def\bd{\bfm d}   \def\bD{\bfm D}  \def\DD{\mathbb{D}}
\def\be{\bfm e}   \def\bE{\bfm E}  \def\EE{\mathbb{E}}
\def\bff{\bfm f}  \def\bF{\bfm F}  \def\FF{\mathbb{F}}
\def\bg{\bfm g}   \def\bG{\bfm G}  \def\GG{\mathbb{G}}
\def\bh{\bfm h}   \def\bH{\bfm H}  \def\HH{\mathbb{H}}
\def\bi{\bfm i}   \def\bI{\bfm I}  \def\II{\mathbb{I}}
\def\bj{\bfm j}   \def\bJ{\bfm J}  \def\JJ{\mathbb{J}}
\def\bk{\bfm k}   \def\bK{\bfm K}  \def\KK{\mathbb{K}}
\def\bl{\bfm l}   \def\bL{\bfm L}  \def\LL{\mathbb{L}}
\def\bm{\bfm m}   \def\bM{\bfm M}  \def\MM{\mathbb{M}}
\def\bn{\bfm n}   \def\bN{\bfm N}  \def\NN{\mathbb{N}}
\def\bo{\bfm o}   \def\bO{\bfm O}  \def\OO{\mathbb{O}}
\def\bp{\bfm p}   \def\bP{\bfm P}  \def\PP{\mathbb{P}}
\def\bq{\bfm q}   \def\bQ{\bfm Q}  \def\QQ{\mathbb{Q}}
\def\br{\bfm r}   \def\bR{\bfm R}  \def\RR{\mathbb{R}}
\def\bs{\bfm s}   \def\bS{\bfm S}  \def\SS{\mathbb{S}}
\def\bt{\bfm t}   \def\bT{\bfm T}  \def\TT{\mathbb{T}}
\def\bu{\bfm u}   \def\bU{\bfm U}  \def\UU{\mathbb{U}}
\def\bv{\bfm v}   \def\bV{\bfm V}  \def\VV{\mathbb{V}}
\def\bw{\bfm w}   \def\bW{\bfm W}  \def\WW{\mathbb{W}}
\def\bx{\bfm x}   \def\bX{\bfm X}  \def\XX{\mathbb{X}}
\def\by{\bfm y}   \def\bY{\bfm Y}  \def\YY{\mathbb{Y}}
\def\bz{\bfm z}   \def\bZ{\bfm Z}  \def\ZZ{\mathbb{Z}}


\def\calA{{\cal  A}} \def\cA{{\cal  A}}
\def\calB{{\cal  B}} \def\cB{{\cal  B}}
\def\calC{{\cal  C}} \def\cC{{\cal  C}}
\def\calD{{\cal  D}} \def\cD{{\cal  D}}
\def\calE{{\cal  E}} \def\cE{{\cal  E}}
\def\calF{{\cal  F}} \def\cF{{\cal  F}}
\def\calG{{\cal  G}} \def\cG{{\cal  G}}
\def\calH{{\cal  H}} \def\cH{{\cal  H}}
\def\calI{{\cal  I}} \def\cI{{\cal  I}}
\def\calJ{{\cal  J}} \def\cJ{{\cal  J}}
\def\calK{{\cal  K}} \def\cK{{\cal  K}}
\def\calL{{\cal  L}} \def\cL{{\cal  L}}
\def\calM{{\cal  M}} \def\cM{{\cal  M}}
\def\calN{{\cal  N}} \def\cN{{\cal  N}}
\def\calO{{\cal  O}} \def\cO{{\cal  O}}
\def\calP{{\cal  P}} \def\cP{{\cal  P}}
\def\calQ{{\cal  Q}} \def\cQ{{\cal  Q}}
\def\calR{{\cal  R}} \def\cR{{\cal  R}}
\def\calS{{\cal  S}} \def\cS{{\cal  S}}
\def\calT{{\cal  T}} \def\cT{{\cal  T}}
\def\calU{{\cal  U}} \def\cU{{\cal  U}}
\def\calV{{\cal  V}} \def\cV{{\cal  V}}
\def\calW{{\cal  W}} \def\cW{{\cal  W}}
\def\calX{{\cal  X}} \def\cX{{\cal  X}}
\def\calY{{\cal  Y}} \def\cY{{\cal  Y}}
\def\calZ{{\cal  Z}} \def\cZ{{\cal  Z}}

%--------------------------------
%
%  Boldfaces in Greek
%
\newcommand{\bfsym}[1]{\ensuremath{\boldsymbol{#1}}}

\def\balpha{\bfsym \alpha}
\def\bbeta{\bfsym \beta}
\def\bgamma{\bfsym \gamma}             \def\bGamma{\bfsym \Gamma}
\def\bdelta{\bfsym {\delta}}           \def\bDelta {\bfsym {\Delta}}
\def\bfeta{\bfsym {\eta}}              \def\bfEta {\bfsym {\Eta}}
\def\bmu{\bfsym {\mu}}                 \def\bMu {\bfsym {\Mu}}
\def\bnu{\bfsym {\nu}}
\def\btheta{\bfsym {\theta}}           \def\bTheta {\bfsym {\Theta}}
\def\beps{\bfsym \varepsilon}          \def\bEps{\bfsym{\mathcal E}}
\def\bepsilon{\bfsym \varepsilon}
\def\bve{\bfsym \varepsilon}
\def\bsigma{\bfsym \sigma}             \def\bSigma{\bfsym \Sigma}
\def\blambda {\bfsym {\lambda}}        \def\bLambda {\bfsym {\Lambda}}
\def\bomega {\bfsym {\omega}}          \def\bOmega {\bfsym {\Omega}}
\def\brho   {\bfsym {\rho}}
\def\btau{\bfsym {\tau}}
\def\bxi{\bfsym {\xi}}          \def\bXi{\bfsym {\Xi}}
\def\bzeta{\bfsym {\zeta}}
\def\bpi{\bfsym {\pi}}          \def\bPi{\bfsym {\Pi}}
\def\bphi{\bfsym {\phi}}          \def\bPhi{\bfsym {\Phi}}
\def\bpsi{\bfsym {\psi}}          \def\bPsi{\bfsym {\Psi}}

%--------------------------------
%
%  Hat (boldface) in Greek
%
\def\halpha{\hat{\alpha}}              \def\hbalpha{\hat{\bfsym \alpha}}
\def\hbeta{\hat{\beta}}                \def\hbbeta{\hat{\bfsym \beta}}
\def\hgamma{\hat{\gamma}}              \def\hgamma{\hat{\bfsym \gamma}}
\def\hGamma{\hat{ \Gamma}}             \def\hbGamma{\hat{\bfsym \Gamma}}
\def\hdelta{\hat{\delta}}              \def\hbdelta{\hat{\bfsym {\delta}}}
\def\hDelta {\hat{\Delta}}             \def\hbDelta{\hat{\bfsym {\Delta}}}
\def\heta{\hat {\eta}}                 \def\hbfeta {\hat{\bfsym {\eta}}}
\def\hmu{\hat{\mu}}                    \def\hbmu {\hat{\bfsym {\mu}}}
\def\hnu{\hat{\nu}}                    \def\hbnu {\hat{\bfsym {\nu}}}
\def\htheta{\hat {\theta}}             \def\hbtheta {\hat{\bfsym {\theta}}}
\def\hTheta{\hat {\Theta}}             \def\hbTheta {\hat{\bfsym {\Theta}}}
\def\hbeps{\hat{\bfsym \varepsilon}}   \def\hbepsilon{\hat{\bfsym \varepsilon}}
\def\hsigma{\hat{\sigma}}              \def\hbsigma{\hat{\bfsym \sigma}}
\def\hSigma{\hat{\Sigma}}              \def\hbSigma{\hat{\bfsym \Sigma}}
\def\hlambda{\hat{\lambda}}            \def\hblambda{\hat{\bfsym \lambda}}
\def\hLambda{\hat{\Lambda}}            \def\hbLambda{\hat{\bfsym \Lambda}}
\def\homega {\hat {\omega}}            \def\hbomega {\hat{\bfsym {\omega}}}
\def\hOmega {\hat {\omega}}            \def\hbOmega {\hat{\bfsym {\Omega}}}
\def\hrho   {\hat {\rho}}              \def\hbrho {\hat{\bfsym {\rho}}}
\def\htau   {\hat {\tau}}              \def\hbtau {\hat{\bfsym {\tau}}}
\def\hxi{\hat{\xi}}                    \def\hbxi{\hat{\bfsym {\xi}}}
\def\hzeta{\hat{\zeta}}                \def\hbzeta{\hat{\bfsym {\bzeta}}}
\def\mE{\mathcal{E}}
\def\ve{\varepsilon}
\def\mF{\mathcal{F}}
\def\mI{{\mathcal  I}}
\def\mG{\mathcal G}
\def\mC{\mathcal C}
\def\mV{\mathcal V}


%--------------------------------
%
%  Operator
%
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\angles}[1]{\left\langle #1 \right\rangle}
\providecommand{\paran}[1]{\left( #1 \right)}
\providecommand{\brackets}[1]{\left[ #1 \right]}
\providecommand{\bbrackets}[1]{\llbracket #1 \rrbracket}
\providecommand{\braces}[1]{\left\{ #1 \right\}}

\providecommand{\convprob}{\stackrel{\calP}{\longrightarrow}}
\providecommand{\convdist}{\stackrel{\calD}{\longrightarrow}}
\providecommand{\defeq}{:=}
%\providecommand{\defeq}{\triangleq}
% \providecommand{\defeq}{\dot{=}}

\usepackage{mathtools}
% K-L divergence
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1 \; \delimsize\| \; #2%
}
\newcommand{\infdiv}{\calD \infdivx}
\newcommand{\kldiv}{\calD_{KL} \infdivx}

%--------------------------------
%
% Regular font in math equation
%

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\corr}{corr}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Dev}{Dev}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\E}{E}
\newcommand{\E}[1]{{\mathbb{E}} \left[ #1 \right]}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\RSS}{RSS}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\SE}{SE}
%\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\matt}{mat}
%\newcommand{\vect}[1]{{\textsc{Vec}} \left( #1 \right)}
%\newcommand{\mat}[1]{{\textsc{Mat}} \left( #1 \right)}

\newtheorem{remark}{Remark}

%--------------------------------
%
%  Bachmann-Landau or asymptotic notations
%
% determiniastic convergence
\newcommand{\bigO}[1]{ \mathcal{O} \left( #1 \right) }
\newcommand{\bigOmega}[1]{ \Omega \left( #1 \right) }
\newcommand{\bigTheta}[1]{ \Theta \left( #1 \right) }
\newcommand{\smlo}[1]{{\rm o} \left( #1 \right) }
\newcommand{\smlomega}[1]{{\omega} \left( #1 \right) }

% converge in probability
\newcommand{\Op}[1]{{\mathcal{O}_p} \left( #1 \right) }
\newcommand{\op}[1]{{\rm o_p} \left( #1 \right) }

\def\cond{\;|\;}

\def\lam {\lambda}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}} % require \usepackage{xcolor}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

\def\aux{\mathrm{src}}
\def\tar{\mathrm{tar}}
\def\ex{\mathrm{e}}
\def\sig{\sigma}
\def\Sig{\Sigma}
\DeclareMathOperator*{\argmax}{arg\,max}

\def\bsig {\bsigma}
\def\bSig {\bSigma}
\def\one {\mathbbm{1}}

\def\eps{\varepsilon}
\def\lam {\lambda}
\def\blam {\blambda}
\def\bLam {\bLambda}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% END: Please put your definitions here:        %%
\def\blue{\color{blue}}
\def\red{\color{red}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{assumption}[theorem]{Assumption}
